Complementary Dynamics

We present a novel approach to enrich arbitrary rig animations with elastodynamic secondary effects. Unlike previous methods which pit rig displacements and physical forces as adversaries against each other, we advocate that physics should complement artists intentions. We propose optimizing for elastodynamic displacements in the subspace orthogonal to displacements that can be created by the rig. This ensures that the additional dynamic motions do not undo the rig animation. The complementary space is high dimensional, algebraically constructed without manual oversight, and capable of rich high-frequency dynamics. Unlike prior tracking methods, we do not require extra painted weights, segmentation into fixed and free regions or tracking clusters. Our method is agnostic to the physical model and plugs into non-linear FEM simulations, geometric as-rigid-as-possible energies, or mass-spring models. Our method does not require a particular type of rig and adds secondary effects to skeletal animations, cage-based deformations, wire deformers, motion capture data, and rigid-body simulations.

==> old-method.tex <==
\begin{wrapfigure}[13]{r}{1.68in}
  \includegraphics[width=\linewidth,trim={6mm 0mm 0mm -10mm}]{fig/orthogonality-notation}
  \label{fig:orthogonality-notation}
\end{wrapfigure} 
%
\section{Method}
Our method adds complementary physical motions to triangle / tetrahedron mesh 
animations obtained using any character rigging process.
%
We start with the most basic setting of our method as a warm-up and 
then introduce the general framework that could be applied to any hyperelastic model and any type of rig parametrization method.
%
We treat different special cases of this general framework as our applications
to show its wide generality and extensibility.\\

FEM-based dynamics dwells in a tetrahedral mesh, while in the traditional animation pipeline the input rig function could operate on both triangle and tetrahedron meshes.
%
To keep everything simple at the beginning, we assume the input to our method is an undeformed tetrahedron mesh in $\R^{d}$ (in 2D reducing to a triangle mesh) with n vertices at rest positions $\V \in \R^{dn}$.
%
Without losing the generality, we treat the rig as a differentiable \emph{rig function} $\u^r : \R^{m} → \R^{dn}$
mapping $m$ \emph{rig parameters} to vertex displacements.
%
Notice that so far we are assuming the codomain of the rig function is the same as our full FEM discretization
i.e. the rig controls every single vertex in the simulation mesh.
%
Or, to put it differently, the animation and simulation meshes are identical.
%
We will show how to deal with it later when those two differ spatially or the rig could only operates on a subset of the tetrahedron mesh.
%
Meanwhile, the physical model to use for the
dynamics is defined by
an elastic potential acting on displacements $E: \R^{dn}
→ \R_{≥0}$ with $E(\mathbf{0}) = 0$ (linear elasticity, mass spring system, ARAP, StVK, neohookean etc).\\
%


% % we don't need this restriction anymore
% We will restrict our consideration to (possibly non-linear) elastic potentials
% that can be written in the form:
% \begin{align}
%   E(\u) = \frac{1}{2}\u^\top \K(\u) \u \text{ with } E(\mathbf{0}) = 0,
% \end{align}
% %
% where $\K : \R^{dn} → \R^{dn×dn}$ maps displacements to a stiffness matrix.


Let us begin by considering the variational form of implicit integration of
Newton's Second Law in the full space of vertex displacements $\u ∈ \R^{dn}$:
%
\begin{align}
%
% \frac{1}{2} \u_t^\top \K(\u_t)
  \label{equ:full-minimization}
  \min_{\u_t} \ \underbrace{E(\u_t)}_\text{potential energy} + \underbrace{\frac{h^2}{2}
  \udd_t^\top \M \udd_t}_\text{momentum term} + \underbrace{-\u_t^\top \f(\u_t)}_\text{work done by external force}
%
\end{align}
%
where $h>0$ is the finite time-step duration, $\M∈\R^{dn×dn}$ is a mass-matrix,
and $\f: \R^{dn}→\R^{dn}$ maps displacements to external forces (impulses,
collisions, wind, drag, etc.).
%
We will use dots to indicate temporal finite
difference of the variable below:
\begin{gather}
  \udd_t := \frac{\ud_t - \ud_{t-1}}{h} \quad \text{ and } \quad
  \ud_t := \frac{\u_t - \u_{t-1}}{h}.
\end{gather}

Our first step is to define the displacements as a sum of dominate rig effects
and secondary physics effects:
%
\begin{align}
  \label{equ:displacements}
  \u_t := \u^r(θ_t) + \u^c_t,
\end{align}
where the rig parameters at time $t$ are given constants and subsequently so are
the rig's contributed displacements $\u^r_{t}$ (we will drop its parameters $θ$
whenever possible), and the unknowns become the \emph{complementary}
displacements $\u^c ∈ \R^{dn}$.

\begin{figure}
  \includegraphics[width=\linewidth]{fig/ballistic-2d}
  \caption{\label{fig:ballistic-2d} 
  \alec{2D example of how adding unconstrained physics will allow ballistic
  motion.}
  }
\end{figure}


\begin{figure}
  \includegraphics[width=\linewidth]{fig/naughty-physics}
  \caption{\label{fig:naughty-physics} 
  \eris{left: rest shape middle: without the additional linear term (original objective) right: with the additional linear term => Artist designs a slender waist but physics tends to make it chubby}
  }
\end{figure}

\begin{figure}
  \includegraphics[width=\linewidth]{fig/daisy}
  \caption{\label{fig:daisy} 
  \eris{same as above}
  }
\end{figure}


This decomposition could be viewed as adding a complementary vector to the original rig input of each frame.
%
However, doing this modification with the objective alone makes no difference with change of variable.
%
Therefore, for these displacements to be truly complementary, we must ensure that $\u^c$
can not manipulate the shape in a way that the rig could have.
%
This would allow the dynamics to \emph{undo} the artist's desires.
%
In the most extreme setting, allowing $\u^c$ to be completely unconstrained 
would allow $\u^c = -\u^r$ so that the elastic potential is always zero: $E(\u^r
+ \u^c) = 0$ (see \reffig{cancel-2d}).
%
Similarly, unconstrained secondary effects would allow a small motion from the
rig to induce ballistic motion of the model (see \reffig{ballistic-2d}).
%
\eris{you mean when having some initial velocity? well didn't quite get this..}
%
There are two criteria we must achieve:
%
\begin{itemize}
  \item no portion of the secondary effects $\u^c$ can be explained by changing
    the rig parameters $θ$, and 
  \item in the absence of external forces and rig \st{acceleration} \eris{velocity}, secondary effects
    \st{are} \eris{should converge to} zero ($\u^c=0$ or equivalently $\u = \u^r$).
\end{itemize}

To achieve the above two criteria, there are two things unique to our complementary dynamics.
%
First, given the artist specified rig parameters for the current time-step $θ_t$,
%
a constraint is introduced to ensure that the
orthogonal projection of $\u_t$ onto the manifold of displacements spanned by the rig
returns the given rig displacement.
%
In the continuous setting, this can be viewed as computing the local integral of the distance between $\u_t$ and the rig manifold $\Y$ over the volumetric domain $\Omega$:
%
\begin{align}
  \argmin_θ \mathlarger{\int_{\Omega}} \left\|  \u_t - \P_{\Y}(\u_t) \right\|^{2} = θ_t.
\end{align}
%
where $\P_{Y}(\u_t)$ denotes the closest-point projection of $\u_t$ onto $\Y$.
%

After the discretization, the integral will be replaced by weighting the 2-norm by a mass matrix $\M$ defined on the tetrahedron mesh:
%
\begin{align}
  \argmin_θ \left\|  \u^r(θ_t) + \u_t^c - \u^r(θ) \right\|_\M² = θ_t.
\end{align}
%

%\begin{figure}
%  \includegraphics[width=0.8\linewidth]{fig/manifold.pdf}
%  \caption{\label{fig:ballistic-2d} 
%    \eris{visualization of the orthogonal constraint}
%  }
%\end{figure}


To first-order, this constraint can be replaced with the simpler linear equality
constraint:
%
\begin{align}
  \label{equ:orthogonality}
  %
  \underbrace{\left.\frac{d \u^r}{d θ}\right|_{θ_t}^\top}_{\A_t^\top}
  \M \u^c_t = \mathbf{0},
\end{align}
%
where $\A_t∈\R^{dn × m}$ is the (known) rig Jacobian matrix evaluated at
$θ_t$.
%
Depending on the rig method to use, $\A_t∈\R^{dn × m}$ can either be a constant matrix
or vary from frame to frame.
%
We use finite difference method (or autodiff) to approximate the Jacobian when the 
analytical solution is not directly available.


The second criteria is motivated by adding just the right force to \emph{cancel}
any elastic potential due to the prescribed rig.
%
To determine this, we start our discussion with linear elasticity material model for simplicity 
i.e. $ E(\u) = \frac{1}{2}\u^\top \K \u $, where $\K$ denotes the constant hessian matrix
(usually stiffness matrix tho) that is positive semi-definite depending on the rest pose only in the linear case.
%
Treat this as a warm up and we will show how this idea could be generalized to any hyperelastic model later.
%
Note that in the absence of external forces and rig velocity,
$\u_t^c$ won't always converge to $\mathbf{0}$ since $\u_t^r$ corresponds to the input 
animation given by the artist who is not aware of dynamics and $\u_t = \u_t^r$ rarely minimizes $E(\u_t)$.
%
This can be annoying sometimes when the rig space is relatively small.
%
In this case physics can be naughty and easily pass the filter to undo what artists are intended to do.
%
As is shown in \reffig{naughty-physics}, artists designs a character to have a slender waist but physics tends to make it chubby,
which corresponds to the pose that has a lower potential energy.
%
Similarly, in \reffig{daisy}, physics is aware of rotating the shape while the artist is simply willing to compress the whole shape.
%
Although there is no ground truth to tell how some rig animation would look like after adding secondary motion,
we claim that the right thing to do is to make artists' consideration the top priority.
%
\eris{not sure how to motivate this second criteria.. maybe we should still treat it as an option for users to decide cuz physics helps to smooth
everything out e.g. fix the candy wrapper artifact etc}
%
Expanding the elastic potential term, we get:
%
\begin{align}
  \frac{1}{2} \u^\top \K \u 
  & = \frac{1}{2} [\u^r + \u^c]^\top \ \K \ [\u^r + \u^c] \\
  & = \frac{1}{2} {\u^c}^\top \K \u^c + {\u^c}^\top
  \underbrace{\K\u^r}_\text{rig force} + \ \text{constant}.
\end{align}


To counteract the contribution of rig force, we add an additional term $- {\u_t^c}^\top\K\u_t^r$ to our original potential energy.
%
Then substituting \refequ{displacements} into the objective of \refequ{full-minimization} results in:
%
\begin{align}
  \underbrace{ \frac{1}{2} {\u_t^c}^\top \K {\u_t^c} }_\text{new potential} + \frac{h^2}{2}
  \udd_t^\top \M \udd_t 
  - \u_t^\top \f(\u_t) + \ \text{constant}.
\end{align}
%
With this new formulation in hand, $\u_t^c$ will eventually converges to $\mathbf{0}$ when there is no external force and rig velocity. This happens because $\K$ is positive semi-definite and also $\u_t^c = \mathbf{0}$ fulfills the constraint proposed in the previous section trivially.

%
Following the discussion above, a direct analogue of rig force appearing in the linear model could be found for nonlinear hyperelastic models.
%
Given any physical model $E: \R^{dn} → \R_{≥0}$, we could add a similar extra term $- {\u_t^c}^\top \nabla E(\u_t^r)$, where $\nabla E(\u_t^r)$ is the corresponding internal elastic force evaluated at $\u_t = \u_t^r$. Then substituting \refequ{displacements} into the objective of \refequ{full-minimization} results in:
%
\begin{align}
  \underbrace{ E(\u_t^r + \u_t^c) - {\u_t^c}^\top\nabla E(\u_t^r) }_\text{new potential} \ + \ \frac{h^2}{2}
  \udd_t^\top \M \udd_t 
  - \u_t^\top \f(\u_t).
\end{align}
%
\\
Let us define the new potential $\widetilde{E}: \R^{dn}
→ \R_{≥0}$ with 
\begin{align}
\widetilde{E}(\u^c_t) = E(\u_t^r + \u_t^c) - {\u_t^c}^\top\nabla E(\u_t^r)
\end{align}
%
whose jacobian and hessian are correspondingly
%
\begin{align}
\nabla \widetilde{E}(\u^c_t) &= \nabla E(\u_t^r + \u_t^c) - \nabla E(\u_t^r)\\
\nabla^2 \widetilde{E}(\u^c_t) &= \nabla^2 E(\u_t^r + \u_t^c)
\end{align}
%
One may notice that $\u_t^c = \mathbf{0}$ is always a saddle point of $\widetilde{E}$ since $\widetilde{E} (\mathbf{0}) = \mathbf{0}$ (first order sufficient condition), and could also be a local minimum when $\nabla^2 E(\u_t^r)$ becomes positive definite (second order sufficient condition).
%
Although there is no guarantee that $\u_t^c = \mathbf{0}$ is a local minimum, we will show it later in the optimization section that $\u_t^c$ could always converge to $\mathbf{0}$.
%
\eris{well..hopefully..}\\

So far we have introduced two things that are specific to our complementary dynamics framework: 1. an orthogonality constraint 2. a modified potential energy by adding one extra rig force term.
%
Since our physical model could be either linear or nonlinear, our rig function could be either linear or nonlinear and the two conditions could be either fully or partially enforced, we demonstrate its wide applications by traversing and instantiating the above combinations, alongside the optimization scheme.\\

Starting with the simplest case, let's consider linear elasticity i.e. $\widetilde{E}(\u^c_t) = \frac{1}{2} {\u_t^c}^\top \K {\u_t^c}$ and linear blend skinning i.e. $\A_{t}$ remains a constant across all the frames. Separating terms and removing constants with respect to the unknowns $\u_t^c$,
we incorporate the orthogonality constraint from \refequ{orthogonality} to
arrive at our complementary dynamics integration optimization:
\begin{align}
  \min_{\u^c_t} & \quad \frac{1}{2} {\u^c_t}^\top \left[ \K +
                \frac{\M}{h^2} \right] \u^c_t \ + \notag \\
                & \quad \quad {\u^c_t}^\top \left[ \M \left[\frac{\u^r_t - \u^r_{t-1}}{h²} -
                \frac{\u^c_{t-1}}{h²} - \frac{\ud_{t-1}}{h} \right] -
                \f(\u_t)\right], \\
  \text{subject to:} & \quad \A^\top \M \u^c_t = \mathbf{0}
\end{align}
%
Since $\K$ is constant, this is a standard quadratic programming problem with a linear constraint.
%
We consider to use Lagrange Multiplier and solve the corresponding KKT system,
whose quadratic part can be prefactored thus ultra fast.
%
The KKT systems says the gradient of Lagrangian should be zero.
%
In matrix form, it is equivalent to
%
\begin{equation}
  \begin{pmatrix}
    \textbf{Q} & \M\A \\
    \A^\top\M & \mathbf{0}\\
  \end{pmatrix}
  %
  \begin{pmatrix}
    \u_t^c \\
    \pmb{\lambda} \\
  \end{pmatrix} 
  =
    \begin{pmatrix}
    \l \\
    \mathbf{0} \\
  \end{pmatrix} 
\end{equation}
%
where
%
\begin{equation}
\begin{split}
\textbf{Q} = \K + \frac{\M}{h^2}
\end{split}
\end{equation}
\begin{equation}
\begin{split}
\l = \M \left[\frac{\u^r_t - \u^r_{t-1}}{h²} -
\frac{\u^c_{t-1}}{h²} - \frac{\ud_{t-1}}{h} \right] -
\f(\u_t)
\end{split}
\end{equation}

%
Notice that $\textbf{Q}$ is sparse and
$\A^\top\M$ is usually dense yet the number of rows is much smaller than the number of columns.
%
Since $\textbf{Q}$ is SPD, we do the following special LU decomposition for $\textbf{Q}$
%
\begin{equation}
  \begin{pmatrix}
    \textbf{Q} & \M\A \\
    \A^\top\M & \mathbf{0}\\
  \end{pmatrix}
  =
  \begin{pmatrix}
    \L & \mathbf{0} \\
    \D^\top & \textbf{B}\\
  \end{pmatrix}
  %
  \begin{pmatrix}
    \L^\top & \D \\
    \mathbf{0} & -\textbf{B}^\top\\
  \end{pmatrix}
\end{equation}
%
where we compute the cholesky factorization $\textbf{Q} = \L \L^\top$, while
$\textbf{D} = \L^{-1} \M\A$ and $\textbf{D}^\top \textbf{D} = \textbf{B} \textbf{B}^\top$
where $\textbf{B}$ is a lower triangular matrix.
%
\eris{copied from alec's thesis. Not sure by how far we should dig into this. Other papers
generally use schur complement.}
\\

\begin{figure}
  \includegraphics[width=\linewidth]{fig/amoeba.pdf}
  \caption{\label{fig:amoeba} 
  \eris{amoeba: single handle + full $\M$ + wind force}
  }
\end{figure}


To cope with the nonlinear models in general,
we approximate the energy in Equation 10 using a second-order Taylor series
in $\u_t^c$, minimize this quadratic function, and iterate
i.e. constrained newton's method as described in \cite{boyd2004convex} to find the optimal solution.
%
We always start from $\u_{i}^c = \mathbf{0}$ which is a feasible point.
%
Then let's look at a single iteration.
%
At this iteration we already have the ith guess of our new complementary displacement,
denoted $\u_{i}^c$.
%
The goal of the $i+1$ iteration is to compute an update in the current velocity estimate
$\Delta \u^c$, that reduces the objective function.
%
This is done by solving a local quadratice optimization problem of the formula
%
\begin{align}
  \Delta {\u^c}^* = 
  \argmin_{\Delta \u^c} & \frac{1}{2} {\Delta \u^c}^\top \H(\u_{i}^c) \Delta \u^c
  + \g(\u_{i}^c)^\top \Delta \u^c \\
  \text{subject to:} & \quad \A^\top \M \Delta \u^c_t = \mathbf{0}.
\end{align}
%
where
%
\begin{align}
  \H &= \M + \frac{\partial^2 E(\u^r + \u_i^c)}{\partial {\u^c}^2}\\
  \g &= \frac{\M}{h^2}(\u^r + \u_i^c - \u_t + h \ud_{t}) - f(\u_t) +
  \frac{\partial E(\u^r + \u_i^c)}{\partial {\u^c}} - \frac{\partial E(\u^r)}{\partial {\u^c}}
  \end{align}
%
In practice people usually apply diagonal Hessian correction for indefinite matrices as described in \cite{nocedal2006numerical}.
%
Hence $\H$ is SPD and the solution of above quadratic optimization problem is given by
$\Delta \u^c = - \H^{-1}\g$. Then update $\u_{i+1}^c = \u_{i}^c + \alpha \Delta \u^c$.
%

\eris{!}
To obtain an optimal step size $\alpha$, we use backtracking line search with Wolfe condition to make sure sufficient decrease
as decribed in \cite{nocedal2006numerical}.
%
However, instead of letting newton run until convergence, we set an upper bound for the total step length.
%
For example, with this upper bound being 1, we set the intial step length to be 0.1 and the maximum number of
iterations to be 10.
%
Empirically, although in general this prevents newton from being convergent, it makes sure
that in the absence of external forces and rig velocity, secondary effects will
converge to zero eventually.
%
The drawback of doing so is that we lose some interesting dynamics due to this not converged newton.
%
\eris{I'm worried this is gonna be our biggest weakness. It's really hard to justify something not converged
could always work.. but that's what I got from experiments :( .}\\

Nevertheless, if we always enforce this orthogonality constraint on every single vertices of the triangle (2D)
or tetrahedron (3D) mesh, there is almost no room for dynamics (completely filtered out).
%
In extreme cases (e.g. linear elasticity), even no dynamics at all (completely adhere to the input animation).
%
Therefore, to achieve interesting secondary motion, one should either rely on proper external forces
(see \reffig{amoeba}) or introduce a fudge factor to redistribute/relax rig forces
(see section 3.9).



%%%%%%% Linear Rig
\subsection{Simple affine rig}
%
A simple yet delightfully useful special case of our formulation happens when
the rig is a single affine transformation:
%
\begin{align}
  \u^r(θ) := \A_\text{single} θ.
\end{align}
where the \emph{constant} matrix $\A_\text{single} ∈ \R^{dn × d(d+1)}$ has the
form:
\begin{align}
  \A_\text{single} = \I_d \otimes 
  \begin{pmatrix}\V_1 & \dots & \V_d & \mathbbm{1} \end{pmatrix}
\end{align}
%
where $\I_d ∈ \R^{d×d}$ is the identity matrix, $\V_i ∈ \R^n$ stacks the $i$th
coordinates of the input vertex positions, and $\mathbbm{1} ∈ \R^{n}$ is a
vector of ones.\\
\\
The rig parameters $θ∈\R^{d(d+1)}$ are the elements of a single affine
transformation matrix controlling the shape. This transformation could be set by
a simple mouse-based user interface, through keyframing, or through an external
procedure e.g. a rigid body simulation.
%
In the 2D amoeba example, the input animation only undergoes rigid transformations and 
we apply some background wind force to achieve interesting motions. See \reffig{amoeba} and the accompanied video.
%
\alec{see cool 2d single-handle example (amoeba)}
\alec{see cool 3d single-handle example (fish?)}

\subsection{Blendshapes}
Blend shapes are commonly used for facial animation and other types of shape interpolation based tasks.
%
For example, in the lcoal delta blendshape formulation,
one face model $\b_0$ (typically the resting face expression)
is designated as the neutral face shape,
while the remaining targets are denotes as $\b_k$.
%
Weight $w_k$ specifies the amount of influence of the k-th face pose.
%
Taking the difference $\b_k - \b_0$ between the k-th face pose
and the neutral face, we get:
%
\begin{align}
  \f = \b_0 + \sum^{n}_{k=1} w_k(\b_k - \b_0)
\end{align}
%
Equivalently, in the matrix form,
%
\begin{align}
  \u_r = \f - \b_0 = \textbf{B}\w
\end{align}
%
Hence in our case, the orthogonality constraint becomes
\begin{align}
\textbf{B} \M \u^c_t = \mathbf{0}
\end{align}
where $\textbf{B}$ formed by displacement vectors is also a constant matrix.
%
\begin{figure}
  \includegraphics[width=0.8\linewidth]{fig/blendshape.pdf}
  \caption{\label{fig:blendshape} 
    \eris{Seungbae's facial animation or the 2D shape interpolation UI?}
  }
\end{figure}

\subsection{Linear blend skinning}
\begin{figure}
  \centering
  \includegraphics[width=0.7\linewidth]{fig/fish}
  \caption{\label{fig:fish}
  \eris{three point handles + linear blend skinning + linear elasticity gold fish (see accompanied video)}
  }
\end{figure}
%
Perhaps the most common rigging method is linear blend skinning (a.k.a. skeletal
subspace deformation).
%
\alec{describe $\A_\text{lbs}$, also constant}
%
Forward/inverse kinematics, mocap, etc.
%
\alec{See cool 2d multi-handle (ginger)}
%
\alec{See cool 3d multi-handle}
%
\alec{See cool 3d skeleton}
%
The user specifies a set of control
handles $\H = \{\h_1, . . . , \h_m\}$, which could be bones of a skeleton,
points or regions on the shape. To deform the shape, the user must specify affine transformations $\T_j ∈ \R^{d × (d+1)}$ for each handle $\h_j$.
%
For each point p on the shape, $\w_j(\p)$ specifies the amount of influence of $\T_j$ on $\p$.
%
The skinning weights are oftern painted manually by specialized rigging
artists, but may also be computed using recent methods automatically.
%
The LBS deformation of the vertices $\textbf{v}_i$ is given by
%
\begin{align}
  \textbf{v}_i^{\prime} = \sum^{m}_{j=1} w_j(\textbf{v}_i) \T_j
  \begin{pmatrix}
    \textbf{v}_i \\
    1 \\
  \end{pmatrix}
\end{align}
%
Or in the equivalent matrix form,
%
\begin{align}
  \textbf{V}^{\prime} = \A_\text{lbs} \T
\end{align}
where $\A_\text{lbs}$ is also a constant matrix. 
%
In the 3D gold fish example, the input animation is controlled by three point handles.%
To realize real-time efficiency, we use linear elasticity model for simplicity.
%
See \reffig{fish} and the accompanied video.


\subsection{Biharmonic Coordinate}
linear.
%
\eris{do we need to describe those one by one? Our contribution doesn't increase by listing those all except for
anything particular. And apparently \cite{hahn2012rig} didn't..}

\subsection{Nonlinear Rig}
%
Wire? DQS?
%
For nonlinear rig functions, we use finite difference method to approximate the Jacobian when the analytic
solution is not directly available.

\subsection{Linear Elasticity}
%
Treat as a warm up. If rig is affine or equivalently $\A$ is constant, then
optimization problem is solved with a linear system that can be prefactored.
%
Small non-rotational displacements.

\subsection{Neohookean}
%
Elasticity research has converged on neohookean.
%
Remember, physics is fast now.
%
Rotation invariant, volume preserving. y.m. and p.r. parameters.
%
Newton's method. Constrain enforced during each solve and line search.

\subsection{Surface only constraint}
It's common that sometimes rig only has control over some certain part of the
input tetrahedron mesh, either directly or indirectly.
%
One typical usecase would be having surface animation as our input and adding 
secondary motion to those surface vertices.
%
In this case we have to introduce the selection matrix based on
barycentric coordinates $\textbf{S}$ which interpolates the tetrahedral deformation
to the surface.
%
Consequently, our orthogonality constraint now becomes
%
\begin{align}
  \argmin_θ \left\|  \u_\text{sur}^r(θ_t) + \textbf{S} \u_t^c - \u_\text{sur}^r(θ) \right\|_{\M_\text{sur}}^2 = θ_t.
\end{align}
%
To first-order, this constraint can be replaced with the simpler linear equality
constraint:
%
\begin{align}
  \label{equ:orthogonality}
  %
  \underbrace{\left.\frac{d \u_{\text{sur}}^r}{d θ}\right|_{θ_t}^\top}_{\A_{\text{sur}}^\top}
  \M_\text{sur} \textbf{S} \u^c_t = \mathbf{0},
\end{align}
%
On the other hand, we have to figure out a way to infer the missing part of $\u_t^r$ as well, since
it also lives on the tetrahedron mesh rather than simply the surface mesh.
%
One way to deal with this is following what has been used in \cite{li2016enriching}.
%
An simpler alternative could be solving a harmonic function over the domain.
%
\begin{align}
  \Delta \u^r & = 1
\end{align}
%
where the input on surface vertices are serving as the boundary condition.
%
Solving the quadratic function with prefactored hessian can be much cheaper than \cite{li2016enriching}.

\eris{surface mass matrix v.s. S * volume mass matrix?}

\subsection{Partial Rig Control / Constraint Relaxation}
Get rid of the boring system and have a fudge factor to generate secondary
motion automatically.
%
See \reffig{constraint}

\begin{figure}
  \includegraphics[width=\linewidth]{fig/constraint}
  \caption{\label{fig:constraint} 
  \eris{illustration of different types of relaxed contraint/fudge factor}
  }
\end{figure}
%
\reffig{constraint} illustrates the idea of having a fudge factor $\mathbf{\Phi}$ to redistribute the rig force over the whole mesh such that
\begin{align}
    \quad \A^\top \mathbf{\Phi} \M \Delta \u^c_t = \mathbf{0}
\end{align}
%
$\mathbf{\Phi}$ is a diagonal matrix with diagonal entries being either 0 or 1. The i-th diagonal entry is equal to 0 when the current vertex is not receiving the orthogonal constraint but 1 otherwise.
%
See the accompanied video for the worm example whose tail is receiving the orthogonality constraint.

\subsection{Fast Mass Springs}
%
Prototypical example of versatile non-continuum based physics. 
%
TRACKS doesn't know what to do with this.
%
Our two augmented criteria doesn't affect the local step.
%
Both the linear term and orthogonal contriant just get add to the global solve.
%
Same for ARAP.

\subsection{Collision Handling}

(no self-collisions, but could be added \cite{BarbicJ10})

%\input{sec/method/1_Objective.tex}
%\input{sec/method/2_QR.tex}
%\input{sec/method/3_Lagrange.tex}
%\input{sec/method/4_AlternativeEnergy.tex}
%\input{sec/method/5_NonlinearModel.tex}



==> sec/method/1_Objective.tex <==
\subsection{Objective and Constraints}
Starting from something simple, we only consider linear blend skinning model and linear elasticity material model for now. The energy model is formulated in the following way: by Newton's second law, we know:
\begin{equation} \label{eq1}
\begin{split}
\textbf{f}_{ext} + \textbf{f}_{int} = \textbf{M}\textbf{a}
\end{split}
\end{equation}
where $\textbf{f}_{ext} \in \mathbb{R}^{dn\times 1}$, $\textbf{f}_{int} \in \mathbb{R}^{dn\times 1}$, $\textbf{M} \in \mathbb{R}^{dn\times dn}$, and $\textbf{a} \in \mathbb{R}^{dn\times 1}$ are the external forces , internal forces, mass matrix and acceleration.\\
Let $V$ denote the potential energy, then
\begin{equation} \label{eq1}
\begin{split}
\textbf{f}_{int} &= -\nabla V\\
\end{split}
\end{equation}
Plug $(2)$ into $(1)$
\begin{equation} \label{eq1}
\begin{split}
\textbf{f}_{ext} - \nabla V &= \textbf{M}\textbf{a}
\end{split}
\end{equation}
For convenience, we write the equation of motion in terms of displacement and let $\textbf{u}_{n+1}$ and $\textbf{v}_{n+1}$ denote the displacement and velocity at time step $n+1$ respectively. Apply the implicit Euler integration scheme and obtain
\begin{equation} \label{eq1}
\begin{split}
\textbf{f}_{ext} - \nabla V(\textbf{u}_{n+1}) &= \textbf{M} \frac{\textbf{v}_{n+1}-\textbf{v}_{n}}{h}\\
\textbf{f}_{ext} - \nabla V(\textbf{u}_{n+1}) &= \textbf{M} \frac{\frac{\textbf{u}_{n+1}-\textbf{u}_{n}}{h}-\textbf{v}_{n}}{h}\\
\textbf{f}_{ext} - \nabla V(\textbf{u}_{n+1}) &= \textbf{M}(\frac{1}{h^2}\textbf{u}_{n+1}-\frac{1}{h^2}\textbf{u}_{n}-\frac{1}{h}\textbf{v}_{n})
\end{split}
\end{equation}
where $h$ is the time step.\\
Take the anti-derivative with respect to $\textbf{u}_{n+1}^{T}$ and we end up with the variational form
\begin{multline*} \label{eq1}
E(\textbf{u}_{n+1}) = \frac{h^2}{2}(\frac{1}{h^2}\textbf{u}_{n+1}-\frac{1}{h^2}\textbf{u}_{n}-\frac{1}{h}\textbf{v}_{n})^{T}\textbf{M}(\frac{1}{h^2}\textbf{u}_{n+1}-\frac{1}{h^2}\textbf{u}_{n}-\frac{1}{h}\textbf{v}_{n})\\
-\textbf{u}_{n+1}^{T}\textbf{f}_{ext}+V(\textbf{u}_{n+1})
\end{multline*}
Note that solving the above update equation (4) is equivalent to solving the optimization problem
\begin{equation} \label{eq1}
\begin{split}
\textbf{u}_{n+1} = \arg\min_{\textbf{u}_{n+1}}E(\textbf{u}_{n+1})
\end{split}
\end{equation}
Following that, assuming using linear elasticity material model and linear tetrahedrons (FEM), we have
\begin{equation} \label{eq1}
\begin{split}
V(\textbf{u}_{n+1}) = \frac{1}{2}\textbf{u}_{n+1}^T\textbf{K}\textbf{u}_{n+1}
\end{split} 
\end{equation}
where $\textbf{K} \in \mathbb{R}^{dn \times dn}$ denotes the global stiffness matrix\\
Plug (7) into (6) and combine similar terms, and then we get
\begin{multline*} \label{eq1}
E(\textbf{u}_{n+1}) = \frac{1}{2h^2}\textbf{u}_{n+1}^T(\textbf{M}+h^2\textbf{K})\textbf{u}_{n+1}+\textbf{u}_{n+1}^T\textbf{M}(-\frac{1}{h^2}\textbf{u}_{n}-\frac{1}{h}\textbf{v}_{n})\\
-\textbf{u}_{n+1}^{T}\textbf{f}_{ext}+const
\end{multline*}
In terms of rigging, assuming using linear blend skinning model, we do the following substitution
\begin{equation} \label{eq1}
\begin{split}
\textbf{u}_{n+1} = (\textbf{A}\textbf{T}_{n+1}-\textbf{X}_0)+(\textbf{u}_{e})_{n+1}
\end{split}
\end{equation}
where $\textbf{A} \in \mathbb{R}^{dn \times (d(d+1)m)}$ is the linear blend skinning matrix combining rest-pose vertex positions $\textbf{X}_0$ with vertex weights and $\textbf{T} \in \mathbb{R}^{(d(d+1)m) \times 1}$ stacks transposed transformation matrices ($d$ presents the dimension of the space and $m$ presents the number of handles) and $(\textbf{u}_{e})_{n+1}$ is the vector that lives in the exterior rig space, which means
\begin{equation} \label{eq1}
\begin{split}
(\textbf{u}_{e})_{n+1}^{T}(\textbf{A}\textbf{S}) = \textbf{0}\quad \forall \textbf{S} \in \mathbb{R}^{(d(d+1)m) \times 1} 
\end{split}
\end{equation}
Since the above equation is true with arbitrary $\textbf{S} \in \mathbb{R}^{(d(d+1)m) \times 1} $, we must have
\begin{equation} \label{eq1}
\begin{split}
(\textbf{u}_{e})_{n+1}^{T}\textbf{A} = \textbf{0}
\end{split}
\end{equation}
i.e.
\begin{equation} \label{eq1}
\begin{split}
\textbf{A}^{T}(\textbf{u}_{e})_{n+1} = \textbf{0}
\end{split}
\end{equation}
which means $(\textbf{u}_{e})_{n+1}$ is living in the right null space of matrix $\textbf{A}^{T}$\\
Plug $(8)$ into the variational equation and combine similar terms and we get the final expression of our quadratic objective function with a linear contraint:
\begin{equation}
\begin{split}
\displaystyle{\minimize_{\textbf{u}_{e}} \ \frac{1}{2}\textbf{u}_{e}^T\textbf{Q}\textbf{u}_{e}+\textbf{u}_{e}^T\textbf{l}}
% \displaystyle{\minimize_{\textbf{u}_{e}} \ E(\textbf{u}_{r}+\textbf{u}_{e})}
\end{split}
\end{equation}
\begin{equation}
\begin{split}
s.t. \ \textbf{A}^{T}\textbf{u}_{e} = \textbf{0}
% s.t. \ \textbf{u}_{e} \in \textbf{W}^{\perp}
\end{split}
\end{equation}
where $\textbf{Q} \in \mathbb{R}^{dn \times dn}$ and $\textbf{l} \in \mathbb{R}^{dn \times 1}$ are constants and
\begin{equation}
\begin{split}
\textbf{Q} &= \frac{1}{h^2}\textbf{M}+\textbf{K}\\
\textbf{l} &= (\frac{1}{h^2}\textbf{M}+\textbf{K})(\textbf{A}\textbf{T}_{n+1}-\textbf{X}_0)-\textbf{M}(\frac{1}{h^2}\textbf{u}_{n}+\frac{1}{h}\textbf{v}_n)-\textbf{f}_{ext}
\end{split}
\end{equation}
where $\textbf{u}_n$ and $\textbf{v}_n$ are vertex positions and velocities from the last time step. Hence for the time step $n+1$, we conclude
\begin{equation}
\begin{split}
\textbf{X}_{n+1} = \textbf{A}\textbf{T}_{n+1}+\displaystyle{\arg\min_{\textbf{u}_{e}} \ (\frac{1}{2}\textbf{u}_{e}^T\textbf{Q}\textbf{u}_{e}+\textbf{u}_{e}^T\textbf{l}})
\end{split}
\end{equation}

==> sec/method/2_QR.tex <==
\subsection{Constraint Elimination}
In terms of how to solve the above quadratic programming problem, the most straightforward approach is to eliminate the constraint by parametrization and convert it into an unconstrained optimization problem. In our case, we could get rid of $\textbf{A}^{T}\textbf{u}_{e} = \textbf{0}$ by presenting $\textbf{u}_{e}$ in the right null space of $\textbf{A}^{T}$. Specifically, with the help of QR decomposition, we could get
\begin{equation}
\textbf{A}^T =
  \begin{bmatrix}
    \textbf{Q}_1 & \textbf{N}
  \end{bmatrix}
  %
  \begin{bmatrix}
    \textbf{R}_1 \\
    \textbf{0} \\
  \end{bmatrix} 
\end{equation}
where $\textbf{N}$ is a basis for the right null space of $\textbf{A}^T$, then we could introduce a new variable $\textbf{y}$, substitute $\textbf{u}_e$ with $\textbf{N}\textbf{y}$ and obtain an unconstrained optimization problem
\begin{equation}
\begin{split}
\displaystyle{\minimize_{\textbf{y}} \frac{1}{2}(\textbf{N}\textbf{y})^T\textbf{Q}(\textbf{N}\textbf{y})+(\textbf{N}\textbf{y})^T\textbf{l}}
\end{split}
\end{equation}
i.e.
\begin{equation}
\begin{split}
\displaystyle{\minimize_{\textbf{y}} \frac{1}{2}\textbf{y}^T\textbf{N}^T\textbf{Q}\textbf{N}\textbf{y}+\textbf{y}^T\textbf{N}^T\textbf{l}}
\end{split}
\end{equation}

==> sec/method/3_Lagrange.tex <==
\subsection{Lagrange Multipliers}
Another way to solve this quadratic programming problem is to use Lagrange Multiplier and sovle the corresponding KKT system. Since ours is a equality-constrained one, the KKT conditions says the gradient of 
\begin{equation}
\begin{split}
L(\textbf{u}_e) = \phi(\textbf{u}_e)+\pmb{\lambda}^T\textbf{A}^T\textbf{u}_e
\end{split}
\end{equation}
should be zero. In matrix form, the KKT system
\begin{equation}
  \begin{bmatrix}
    \textbf{H} & \textbf{A}\\
    \textbf{A}^T & \textbf{0}\\
  \end{bmatrix}
  %
  \begin{bmatrix}
    \textbf{u}_e \\
    \pmb{\lambda} \\
  \end{bmatrix}
  =
    \begin{bmatrix}
    \textbf{d} \\
    \textbf{0} \\
  \end{bmatrix} 
\end{equation}
where
\begin{equation}
\begin{split}
\textbf{H} = \frac{1}{h^2}\textbf{M}+\textbf{K}
\end{split}
\end{equation}
\begin{equation}
\begin{split}
\textbf{d} = (\frac{1}{h^2}\textbf{M}+\textbf{K})(\textbf{A}\textbf{T}_{n+1}-\textbf{X}_0)-\textbf{M}(\frac{1}{h^2}\textbf{u}_{n}+\frac{1}{h}\textbf{v}_n)-\textbf{f}_{ext}
\end{split}
\end{equation}
Then apply direct or indirect methods to solve above linear system e.g. Gauss elimination, $LDL^T$ factorization, newton's method etc.

==> sec/method/4_AlternativeEnergy.tex <==
\subsection{Alternative Energy Formulation}
Consider adding one extra explicit spring force $\textbf{f}_{p} = -\textbf{K}(\textbf{A}\textbf{T}-\textbf{X}_0))$ to the material model
\begin{equation}
\begin{split}
\textbf{K}\textbf{u}+\textbf{f}_{p}+\textbf{M}\ddot{\textbf{u}} = 0\\
\textbf{K}(\textbf{u}_e+(\textbf{A}\textbf{T}-\textbf{X}_0))+\textbf{f}_{p}+\textbf{M}\ddot{\textbf{u}} = 0\\
\textbf{K}(\textbf{u}_e+(\textbf{A}\textbf{T}-\textbf{X}_0))-\textbf{K}(\textbf{A}\textbf{T}-\textbf{X}_0)+\textbf{M}\ddot{\textbf{u}} = 0\\
\textbf{K}\textbf{u}_e+\textbf{M}\ddot{\textbf{u}}=0
\end{split}
\end{equation}
As a result, only the displacement obtained from the exterior space will be considered when measuring the internal force and we ignore the displacement caused by skinning. In this case, $\textbf{f}_{p}$ could be interpreted as plasticity.\\
Generally speaking, if introducing a scalar parameter to control the degree of plasticity i.e. $\textbf{f}_{p} = -p \textbf{K}(\textbf{A}\textbf{T}-\textbf{X}_0))$, then the linear term $\textbf{l}$ in Eqn 13 becomes
\begin{equation}
\begin{split}
\textbf{l} &= (\frac{1}{h^2}\textbf{M}+(1-p)\textbf{K})(\textbf{A}\textbf{T}_{n+1}-\textbf{X}_0)-\textbf{M}(\frac{1}{h^2}\textbf{u}_{n}+\frac{1}{h}\textbf{v}_n)-\textbf{f}_{ext}\\
\end{split}
\end{equation}


==> sec/method/5_NonlinearModel.tex <==
\subsection{Nonlinear Elastodynamics Model}
Our method described above could be easily extended to nonlinear elastodynamics models, where we consider newton's method with equality constraints. Start from the discrete time stepping equation and apply the implicit Euler integration scheme to obtain
\begin{equation}
\begin{split}
\textbf{M}\textbf{v}^{t+1} &= \textbf{M}\textbf{v}^{t} + \Delta t \textbf{f}(\textbf{u}^{t+1})\\
\textbf{M}\textbf{v}^{t+1} &= \textbf{M}\textbf{v}^{t} + \Delta t \textbf{f}(\textbf{u}^{t}+\Delta t \textbf{v}^{t+1})
\end{split}
\end{equation}
Then the equivalent optimization problem is
\begin{equation}
\begin{split}
\textbf{v}^{t+1} = \displaystyle{\arg\min_{\textbf{v}} \ (\frac{1}{2} (\textbf{v}-\textbf{v}^{t})^T\textbf{M}(\textbf{v}-\textbf{v}^{t}) } + V(\textbf{u}^{t}+\Delta t \textbf{v}))
\end{split}
\end{equation}
let $\Delta \textbf{v} = \textbf{v}^{t+1} - \textbf{v}^{t}$ and $\Bar{\textbf{u}} = \textbf{u}^{t}+\Delta t\textbf{v}^{t}$, then
\begin{equation}
\begin{split}
\textbf{v}^{t+1} &= \displaystyle{\arg\min_{\textbf{v}} \ (\frac{1}{2} (\textbf{v}-\textbf{v}^{t})^T\textbf{M}(\textbf{v}-\textbf{v}^{t}) } + V(\textbf{u}^{t}+\Delta t \textbf{v}))\\
\Delta \textbf{v} &= \displaystyle{\arg\min_{\Delta \textbf{v}} \ (\frac{1}{2} \Delta \textbf{v}^T\textbf{M}\Delta \textbf{v} } + V(\textbf{u}^{t}+\Delta t (\textbf{v}^{t}+\Delta \textbf{v})))\\
\Delta \textbf{v} &= \displaystyle{\arg\min_{\Delta \textbf{v}} \ (\frac{1}{2} \Delta \textbf{v}^T\textbf{M}\Delta \textbf{v} } + V((\textbf{u}^{t}+\Delta t \textbf{v}^{t})+\Delta t \Delta \textbf{v}))\\
\Delta \textbf{v} &= \displaystyle{\arg\min_{\Delta \textbf{v}} \ (\frac{1}{2} \Delta \textbf{v}^T\textbf{M}\Delta \textbf{v} } + V(\bar{\textbf{u}}+\Delta t \Delta \textbf{v}))
\end{split}
\end{equation}
To obtain a local quadratic approximation to the objective function, we could do Taylor expansion around $\bar{\textbf{u}}$ up to the second order term
\begin{equation}
\begin{split}
\Delta \textbf{v} &= \displaystyle{\arg\min_{\Delta \textbf{v}} \ (\frac{1}{2} \Delta \textbf{v}^T\textbf{M}\Delta \textbf{v} } + \Delta t \Delta \textbf{v}^{T} \frac{\partial V}{\partial \textbf{u}} \big(\bar{\textbf{u}} \big)+\frac{1}{2}\Delta t^2 \Delta \textbf{v}^{T} \frac{\partial^2 V}{\partial \textbf{u}^{2}}\big(\bar{\textbf{u}} \big) \Delta \textbf{v} )
\end{split}
\end{equation}

\begin{equation}
\begin{split}
\textbf{u}^{t+1} &= \displaystyle{\arg\min_{\textbf{u}} \ (\frac{1}{2} \textbf{u}^T (\frac{\textbf{M}}{\Delta t^{2}}+\textbf{K}) \textbf{u} } +  \textbf{u}^{T} (\frac{\textbf{M}}{\Delta t^{2}}+\textbf{K})(-\textbf{u}^{t} - \Delta t\textbf{v}^{t}) + \textbf{u}^{T}\textbf{f})
\end{split}
\end{equation}
where $\textbf{f} = \frac{\partial V}{\partial \textbf{u}}\big(\bar{\textbf{u}}\big)$ and $\textbf{K} = \frac{\partial^2 V}{\partial \textbf{u}^{2}}\big(\bar{\textbf{u}} \big)$

% \begin{equation}
% \begin{split}
% \Delta \textbf{u}^{*} = \displaystyle{\arg\min_{\Delta \textbf{u}} \ (\frac{1}{2h^2}\Delta \textbf{u}^T\textbf{M}\Delta \textbf{u}-\Delta \textbf{u}^T\textbf{M}\textbf{u}^{t} - \frac{1}{2}\Delta \textbf{u}^T \textbf{K}\Delta \textbf{u} - \frac{1}{h}\Delta \textbf{u}^T \textbf{f} })
% \end{split}
% \end{equation}
% \begin{equation}
% \begin{split}
% \textbf{U} = \textbf{U}_{LBS} + W(\textbf{U}_{LBS})\textbf{U}_{e}
% \end{split}
% \end{equation}

% \begin{multline*}
% E(\textbf{u}^{t+1}) = \frac{h^2}{2}(\frac{1}{h^2}\textbf{u}^{t+1}-\frac{1}{h^2}\textbf{u}^{t}-\frac{1}{h}\textbf{v}^{t})^{T}\textbf{M}(\frac{1}{h^2}\textbf{u}^{t+1}-\frac{1}{h^2}\textbf{u}^{t}-\frac{1}{h}\textbf{v}^{t})\\
% +V(\textbf{u}^{t+1})
% \end{multline*}

